Regret and Belief Complexity Trade-off in Gaussian Process Bandits via Information Thresholding

Bayesian optimization is a framework for global search via maximum a posteriori updates rather than simulated annealing, and has gained prominence for decision-making under uncertainty. In this work, we cast Bayesian optimization as a multi-armed bandit problem, where the payoff function is sampled from a Gaussian process (GP). Further, we focus on action selections via upper confidence bound (UCB) or expected improvement (EI) due to their prevalent use in practice. Prior works using GPs for bandits cannot allow the iteration horizon $T$ to be large, as the complexity of computing the posterior parameters scales cubically with the number of past observations. To circumvent this computational burden, we propose a simple statistical test: only incorporate an action into the GP posterior when its conditional entropy exceeds an $\epsilon$ threshold. Doing so permits us to precisely characterize the trade-off between regret bounds of GP bandit algorithms and complexity of the posterior distributions depending on the compression parameter $\epsilon$ for both discrete and continuous action sets. To best of our knowledge, this is the first result which allows us to obtain sublinear regret bounds while still maintaining sublinear growth rate of the complexity of the posterior which is linear in the existing literature. Moreover, a provably finite bound on the complexity could be achieved but the algorithm would result in $\epsilon$-regret which means $\textbf{Reg}_T/T \rightarrow \mathcal{O}(\epsilon)$ as $T\rightarrow \infty$. Experimentally, we observe state of the art accuracy and complexity trade-offs for GP bandit algorithms applied to global optimization, suggesting the merits of compressed GPs in bandit settings.

==> Experiments2.tex <==
%!TEX root = main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% S  E  C  T  I  O  N %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Experiments}\label{sec:exp}
In this section, we evaluate the performance of the statistical compression method under a few different action selections (acquisition functions). Specifically, Algorithm \ref{alg:cub} employs the Upper Confidence Bound (UCB) or Expected Improvement (EI) \citep{nguyen2017regret} acquisition function, but the key insight here is a modification of the GP posterior, not the action selection. Thus, we validate its use for Most Probable Improvement (MPI) \citep{wang2014theoretical} as well, defined as
%
%
\begin{align}\label{eq:EIMPI}
%\text{\textcolor{blue}{include equations and definitions for EI and MPI}}
\alpha^{\text{MPI}}(\bbx)&=\sigma_{t-1}\phi(z) + [\mu_{t-1}(\bbx) - \xi]\Phi(z)\;, \nonumber \\
\xi&=\argmax_{\bbx} \mu_{t-1}(\bbx) \ \ \nonumber % \\
%\alpha^{\text{EI}}(\bbx)=\sigma_{t-1}\phi(z) + [\mu_{t-1}(\bbx) - \xi]\Phi(z)\;, \xi=\max\{y_u\in\ccalS_{t-1}\} \ \  \nonumber  
\end{align}
%
where $\phi(z)$ and  $\Phi(z)$ denote the standard Gaussian density and distribution functions, and $z=(\mu_{t-1}(\bbx) - \xi)/\sigma_{t-1}(\bbx)$ is the centered $z$-score.
We further compare the compression scheme against Budgeted Kernel Bandits (BKB) proposed by \citep{calandriello2019gaussian} which proposes to randomly add or drop points according to a distribution that is inversely proportional to the posterior variance, also on the aforementioned acquisition functions.

 Unless otherwise specified, the squared exponential kernel is used to represent the correlation between the input, the lengthscale is set to $\theta$ = 1.0, the noise prior is set to $\sigma^2$ = 0.001, the compression budget $\epsilon$ = $10^{-4}$ and the confidence bounds hold with probability of at least $\delta$ = 0.9. As a common practice across all three problems, we initialize the Gaussian priors with $2^{d}$ training data randomly collected from the input domain, where d is the input dimension. We quantify the performance using Mean Average Regret over the iterations and the clock time. In addition, the model order, or number of points defining the GP posterior, is visualized over time to characterize the compression of the training dictionary. To ensure fair evaluations, all the listed simulations were performed on a PC with 1.8 GHz Intel Core i7 CPU and 16 GB memory. Same initial priors and parameters are used to assess computational efficiency in terms of the compression.

 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]\hspace{-1mm}
	\subfigure[UCB]{\includegraphics[width=0.335\linewidth,height=2.6cm]
	                {img1_1.pdf}\label{subfig:xamplUCBmar}}\hspace{-1mm}
	\subfigure[EI]{\includegraphics[width=0.332\linewidth,height=2.6cm]
	                {img2_1.pdf}\label{subfig:xamplEImar}}\hspace{-1mm}
	\subfigure[MPI]{\includegraphics[width=0.335\linewidth,height=2.6cm]
	                {img3_1.pdf}\label{subfig:xamplMPImar}} \vspace{-0mm}\\
	                %
	         \hspace{-1mm}       	\subfigure[UCB]{\includegraphics[width=0.335\linewidth,height=2.6cm]
	                {img7_1.pdf}\label{subfig:xamplUCBCT}}\hspace{-1mm}
	\subfigure[EI]{\includegraphics[width=0.335\linewidth,height=2.6cm]
	                {img8_1.pdf}\label{subfig:xamplEICT}}\hspace{-1mm}
	\subfigure[MPI]{\includegraphics[width=0.335\linewidth,height=2.6cm]
	                {img9_1.pdf}\label{subfig:xamplMPICT}}\vspace{-0mm}\\
	                %
	                	\subfigure[UCB]{\includegraphics[width=0.335\linewidth,height=2.6cm]
	                {img4_1.pdf}\label{subfig:xamplUCBM}}\hspace{-1mm}
	\subfigure[EI]{\includegraphics[width=0.335\linewidth,height=2.6cm]
	                {img5_1.pdf}\label{subfig:xamplEIM}}\hspace{-1mm}
	\subfigure[MPI]{\includegraphics[width=0.335\linewidth,height=2.6cm]
	                {img6_1.pdf}\label{subfig:xamplMPIM}}\vspace{-0mm}
%
    \caption{We display mean average regret vs iteration (top row) and clock time (middle row) for the proposed algorithm with uncompressed and BKB variants on the {\bf example function} for various acquisition functions. Observe that our proposed compression scheme attains comparable regret to the dense GP. Moreover, the associated model complexity of the GP settles to an intrinsic constant discerned by the learning process (bottom row), as compared with alternatives which either randomly vary, or grow unbounded.}\label{fig:xampl1}
    \vspace{-4mm}
\end{figure} 
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{table}[t]
\centering
\begin{tabular}{||c c c c ||} 
 \hline
 Acquisition & Uncompressed & Compressed & BKB \\ [0.5ex] 
 \hline\hline
 UCB & 6.756 & \textbf{5.335} & 9.56 \\ 
 EI & 7.594 & \textbf{4.133} & 10.578 \\
 MPI & 5.199 & \textbf{3.864} & 9.429\\ [1ex] 
 \hline
\end{tabular}
\caption{Clock Times (in seconds) with example function}
\label{table:xampl}
\vspace{-0mm}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Example function}\label{subsec:xampl}
Firstly, we evaluate our proposed method on an example function given by Equation \ref{eq:xampl}
\begin{equation}\label{eq:xampl}
    f(x) = \sin(x)  +  \cos(x)  +  0.1\times x
\end{equation}

A random Gaussian noise is induced at every observation of f, to emulate the practical applications of Bayesian Optimization where the black box functions are often corrupted by noise. 

The results of this experiment are shown in Figure \ref{fig:xampl1}, and the associated wall clock times are demonstrated in Table \ref{table:xampl}. Observe that the compression rule \eqref{eq:compression_rule} yields regret that is typically comparable to the dense GP, with orders of magnitude reduction in model complexity. This complexity reduction, in turn, permits a state of the art tradeoff in regret versus wall clock time for certain acquisition functions, i.e., the UCB and EI, but not MPI. Interestingly, the model complexity of Algorithm \ref{alg:cub} settles to a constant discerned by the covering number (metric entropy) of the action space, validating the conceptual result of Theorem \ref{model_order}.


%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Rosenbrock Function}\label{subsec:rosen}

For the second experiment, we compare the compressed variants with their baseline algorithm on a two-dimensional non-convex function popularly known as the Rosenbrock Function, given by:
%
\begin{equation}\label{eq:rosen}
    f(x, y) = (a-x)^2  +  b(y - x^2)^2
\end{equation}
%
The Rosenbrock function is a common benchmark non-convex function used to validate the performance of global optimization methods. Here we set its parameters as $a=1$ and $b=10$ for simplicity throughout. Again, we run various (dense and reduced-order) Gaussian Process bandit algorithms with different acquisition functions. 

The results of this experiment are displayed in Figure \ref{fig:rosen} with associated wall clock times collected in Table \ref{table:rosen}. Again, we observe that compression with respect to conditional entropy yields a minimal reduction in performance in terms of regret while translating to a significant reduction of complexity. Specifically, rather than growing linearly with the number of past actions, as is standard in nonparametric statistics, the model order settles down to an intrinsic constant determined by the metric entropy of the action space. This means that we obtain a state of the art tradeoff in model complexity versus regret, as compared with the dense GP or probabilistic dropping inversely proportional to the variance, as in \citep{calandriello2019gaussian}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]\hspace{-1mm}
	\subfigure[UCB]{\includegraphics[width=0.335\linewidth,height=2.8cm]
	                {img1_2.pdf}\label{subfig:rosenUCBmar}}\hspace{-1mm}
	\subfigure[EI]{\includegraphics[width=0.332\linewidth,height=2.8cm]
	                {img2_2.pdf}\label{subfig:rosenEImar}}\hspace{-1mm}
	\subfigure[MPI]{\includegraphics[width=0.335\linewidth,height=2.8cm]
	                {img3_2.pdf}\label{subfig:rosenMPImar}} \vspace{-1mm}\\
	                %
	         \hspace{-1mm}       	\subfigure[UCB]{\includegraphics[width=0.335\linewidth,height=2.8cm]
	                {img7_2.pdf}\label{subfig:rosenUCBCT}}\hspace{-1mm}
	\subfigure[EI]{\includegraphics[width=0.335\linewidth,height=2.8cm]
	                {img8_2.pdf}\label{subfig:rosenEICT}}\hspace{-1mm}
	\subfigure[MPI]{\includegraphics[width=0.335\linewidth,height=2.8cm]
	                {img9_2.pdf}\label{subfig:rosenMPICT}}\vspace{-1mm}\\
	                %
	                	\subfigure[UCB]{\includegraphics[width=0.335\linewidth,height=2.8cm]
	                {img4_2.pdf}\label{subfig:rosenUCBM}}\hspace{-1mm}
	\subfigure[EI]{\includegraphics[width=0.335\linewidth,height=2.8cm]
	                {img5_2.pdf}\label{subfig:rosenEIM}}\hspace{-1mm}
	\subfigure[MPI]{\includegraphics[width=0.335\linewidth,height=2.8cm]
	                {img6_2.pdf}\label{subfig:rosenMPIM}}\vspace{-1mm}
    \caption{We display mean average regret vs iteration (top row) and clock time (middle row) for the proposed algorithm with uncompressed and BKB variants on the {\bf Rosenbrock function} for various acquisition functions. The compression based on conditional entropy yields  regret to comparable to the dense GP, with an associated model order that settles to a constant extracted by the optimization process (bottom row), as compared with alternatives which either randomly vary, or grow unbounded.}\label{fig:rosen}\vspace{-0cm}
\end{figure} 
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\begin{tabular}{||c c c c ||} 
 \hline
 Acquisition & Uncompressed & Compressed & BKB \\ [0.5ex] 
 \hline\hline
 UCB & 2.412 & \textbf{1.905} & 3.143\\ 
 EI & 2.604 & \textbf{2.246}  & 3.801\\
 MPI & 2.533 & \textbf{2.186} & 3.237\\ [1ex] 
 \hline
\end{tabular}
\caption{Clock Times (in seconds) on the Rosenbrock}
\label{table:rosen}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Hyper-paramter Tuning in Logistic Regression}\label{subsec:mnist}
In this subsection, we propose using bandit algorithms to automate the hyper-parameter tuning of machine learning algorithms. More specifically, we propose using Algorithm \ref{alg:cub} and variants with different acquisition functions to tune the following hyper-parameters of a supervised learning scheme, whose concatenation forms the action space: the learning rate, batch size, dropout of the inputs, and the $\ell_2$ regularization constant. The specific supervised learning problem we focus on is the training of a multi-class logistic regressor over the MNIST training set \cite{lecun} for classifying hand written digits. The instantaneous reward here is the statistical accuracy on a hold-out validation set. 
\begin{table}[h]
\centering
\begin{tabular}{||c c c c ||} 
 \hline
 Acquisition & Uncompressed & Compressed & BKB \\ [0.5ex] 
 \hline\hline
 UCB & 5.18 & \textbf{5.288} & 4.836 \\ 
 EI & 5.948 & \textbf{5.611} & 4.82  \\
 MPI & 5.642 & \textbf{4.99} & 4.867 \\  [1ex] 
 \hline
\end{tabular}
\caption{Clock Times (in seconds) with Hyperparameter Tuning}
\label{table:mnist}
\end{table}
Considering the high-dimensional input domain and the number of training examples, GP dictionary may explode to a large size. In large-scale settings, the input space could be much larger with many more hyper-parameters to tune, in which case GPs may be computationally intractable.  The statistical compression proposed here ameliorates this issue by keeping the size of training dictionary in check, which makes it feasible for hyper-parameter tuning as the number of training examples becomes large. 

The results of this implementation are given in Figure \ref{fig:mnist} with associated compute times in Table \ref{table:mnist}. Observe that the trend identified in the previous two examples translates into practice here: the compression technique \eqref{eq:compression_rule} yields algorithms whose regret is comparable to the dense GP, with a significant reduction in model complexity that eventually settles to a constant. This constant is a fundamental measure of the complexity of the action space required for finding a no-regret policy. Overall, then, one can run Algorithm \ref{alg:cub} on the back-end of any training scheme for supervised learning in order to automate the selection of hyper-parameters in perpetuity without worrying about eventual slowdown.




==> Introduction_Conflict_.tex <==
%%
%!TEX root = main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% S  E  C  T  I  O  N %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Introduction}

Bayesian optimization is a framework for global optimization of a black box function via noisy evaluations \citep{frazier2018tutorial}, and provides an alternative to simulated annealing \citep{kirkpatrick1983optimization,bertsimas1993simulated} or exhaustive search \citep{davis1991handbook}. These methods have proven adept at hyper-parameter tuning of machine learning models \citep{snoek2012practical,li2017hyperband}, nonlinear system identification \citep{srivastava2013optimal}, experimental design \citep{chaloner1995bayesian,press2009bandit}, and semantic mapping \citep{shotton2008semantic}.


More specifically, denote the function $f: \ccalX \rightarrow \reals $ we seek to optimize through noisy samples, i.e., for a given choice $\bbx_t\in\ccalX$, we observe $y_t = f(\bbx_t) + \epsilon_t$ sequentially. We make no assumptions for now on the convexity, smoothness, or other properties of $f$, other than each function evaluation must be selected judiciously. 
%
Our goal is to select a sequence of actions $\{\bbx_t\}$ that eventuate in competitive performance with respect to the optimal selection $\bbx^*=\argmax_{\bbx \in \ccalX} f(\bbx)$. For sequential decision making, a canonical performance metric is \emph{regret}, which quantifies the performance of a sequence of decisions $\{\bbx_t\}$ as compared with the optimal action $\bbx^*$:
%
\begin{equation}\label{eq:regret}
%
\textbf{Reg}_T:=\sum_{t=1}^T (f(\bbx^*) - f(\bbx_t)).
%
\end{equation}
%
Regret in \eqref{eq:regret} is natural because at each time we quantify how far decision $\bbx_t$ was from optimal through the difference $r_t:=f(\bbx^*) - f(\bbx_t)$. An algorithm eventually learns the optimal strategy if it is no-regret: $\textbf{Reg}_T/T \rightarrow 0$ as $T\rightarrow \infty$.

In this work, we focus on Bayesian settings in which a likelihood model is hypothesized to relate the unknown function $f(\bbx)$ and action selection $\bbx\in\ccalX$. Then upon selecting an action $\bbx$, one tracks a posterior distribution, or \emph{belief model} \citep{powell2012optimal}, over possible outcomes $y=f(\bbx) + \epsilon$ which informs how the next action is selected. In classical Bayesian inference, posterior distributions do not influence which samples $(\bbx, y)$ are observed next \citep{ghosal2000convergence}. In contrast, in multi-armed bandits, action selection $\bbx$ determines which observations form the posterior, which is why it is also referred to as \emph{active learning} \citep{jamieson2015next}. 

Two key questions in this setting are how to specify a (i) likelihood and (ii) action selection strategy. These specifications come with their own merits and drawbacks in terms of optimality and computational efficiency. Regarding (i) the likelihood model, when the action space $\ccalX$ is discrete and of moderate size $X=|\ccalX|$, one may track a probability for each element of $\ccalX$, as in Thompson (posterior) sampling \citep{russo2018tutorial}, Gittins indices \citep{gittins2011multi}, and the Upper Confidence Bound (UCB) \citep{auer2002nonstochastic}. These methods differ in their manner of action selection, but not distributional representation. 

 However, when the range of possibilities $X$ is large, computational challenges arise. This is because the number of parameters one needs to define a posterior distribution over $\ccalX$ is proportional to $X$, an instance of the curse of dimensionality in nonparametric statistics. One way to circumvent this issue for continuous spaces is to discretize the action space according to a pre-defined time-horizon that determines the total number of selected actions \citep{bubeck2011lipschitz,magureanu2014lipschitz}, and carefully tune the discretization to the time-horizon $T$. The drawback of these approaches is that as $T\rightarrow \infty$, the number of parameters in the posterior grows intractably large.
 
 An alternative is to define a history-dependent distribution directly over the large (possibly continuous) space using, e.g., Gaussian Processes (GPs) \citep{rasmussen2004gaussian} or Monte Carlo (MC) methods \citep{smith2013sequential}. Bandit action selection strategies based on such distributional representations have been shown to be no-regret in recent years -- see   \citep{srinivas2012information,gopalan2014thompson}. While MC methods permit the most general priors on the unknown function $f$, computational and technical challenges arise when the prior/posterior no longer posses conjugacy properties \citep{gopalan2014thompson}.  By contrast, GPs, stochastic processes with any finite collection of realizations of which are jointly Gaussian \citep{krige1951statistical}, have a conjugate prior and posterior, and thus their parametric updates admit a closed form -- see  \citep{rasmussen2004gaussian}[Ch. 2]. 
 
 The conjugacy of the GP prior and posterior has driven its use in bandit action selection. In particular, by connecting regret to maximum information-gain based exploration, which upper-bounds the posterior variance \citep{srinivas2012information,de2012exponential}, no-regret algorithms may be derived through variance maximization. Doing so yields actions which over-prioritize exploration, which may be balanced through, e.g., upper-confidence bound (UCB) based action selection. GP-UCB algorithms, and variants such as expected improvement (EI) \citep{wang2014theoretical,nguyen2017regret}, and step-wise uncertainty reduction (SUR) \citep{villemonteix2009informational}, including knowledge gradient \citep{frazier2008knowledge}, have been shown to be no-regret or statistically consistent \citep{bect2019supermartingale}  in recent years.
 

 
However, these convergence results hinge upon requiring use of the dense GP whose posterior distribution [cf. \eqref{eq:posterior_parameters}], has complexity cubic in $T$ due to the inversion of a Gram (kernel) matrix formed from the entire training set. Hence, the major limiting factor associated with the use of GP-UCB algorithm in practice is its computational cost. For a given $|\mathcal{X}|$ number of actions (finite decision set) to choose from, GP-UCB algorithm exhibit $\mathcal{O}(|\mathcal{X}|T^2)$ per step runtime and $\mathcal{O}(|\mathcal{X}|T)$ space (memory) complexity for each new decision when run for a time horizon of length $T$. Numerous efforts to reduce the complexity of GPs exist in the literature -- see \citep{csato2002sparse,bauer2016understanding,bui2017streaming}. These methods all fix the complexity of the posterior and ``project" all additional points onto a fixed likelihood ``subspace." Doing so, however, may cause uncontrollable statistical bias and divergence. In \cite{calandriello2019gaussian}, by the proposing to use a number of inducing points of the order of effective dimension  $\mathcal{O}(d_{\text{eff}})$, one may reduce the complexity to $\mathcal{O}(|\mathcal{X}|d_{\text{eff}}^2)$ and $\mathcal{O}(|\mathcal{X}|d_{\text{eff}})$ for per step runtime and space complexity, respectively. However, the effective dimension  $d_{\text{eff}}$ cannot be computed in advance of runtime due to its dependence on a $T\times T$ Gram matrix of kernel evaluations, which makes selection of the number of inducing inputs an open problem that may be partially solved via multiple training epochs \citep{calandriello2020near}. Contemporaneous work has established the effectiveness of greedy approximation of RKHS elements in the bandit setting \citep{takemori2020approximation}, but considers function space norms as the approximation criteria. Instead, here, we directly tune the approximation to the information-theoretic notion of regret.

More specifically, we explicitly design approximate GPs to ensure both small regret and moderate complexity. This goal is obtained by putting forth a compression metric based upon the conditional entropy of an action. That is, we retain actions in the GP representation whose conditional entropy exceeds an $\epsilon$-threshold. Doing so then allows us to come up with on-the-fly dynamically adjusted GP representations whose per step runtime is  $\mathcal{O}(|\mathcal{X}|T)$  and requires storing $\mathcal{O}(|\mathcal{X}|\sqrt{T})$ points via selection of  the compression metric as $\epsilon=\mathcal{O}(1/\sqrt{T})$.\footnote{These dynamically self-adjusting nonparametric density estimates have recently been studied for estimation and regression in, e.g., \citep{koppel2019consistent,elvira2016adapting}.  } Importantly, one may select $\epsilon$ simply to be any positive (and often small) constant in practice, and hence does not depend oracle knowledge of the Gram matrix of kernel evaluations as in \cite{calandriello2019gaussian,calandriello2020near}. Overall, then, our main contributions are as follows:
%
\begin{itemize}
%
\item we propose a statistical test that operates inside GP-UCB or GP-EI which incorporates actions into the GP posterior only when conditional entropy exceeds an $\epsilon$ threshold (Sec. \ref{sec:prob}). We call these methods Compressed GP-UCB or Compressed GP-EI (Algorithm \ref{alg:cub}).
%
\item derive sublinear regret bounds of GP bandit algorithms up to factors depending on the compression parameter $\epsilon$ for both discrete and continuous action sets (Sec. \ref{sec:convergence}). 
%
\item establish that the complexity of the GP posterior remains provably finite and depends on the Shannon Capacity of the observation space  (Sec. \ref{sec:convergence}). 
%
\item experimentally employ these approaches for optimizing non-convex functions and tuning the regularizer and step-size of a logistic regressor, which obtains a state of the art trade off in regret versus computational efficiency relative to a few baselines \citep{srinivas2012information,calandriello2019gaussian}.  (Sec. \ref{sec:exp}). 
 \end{itemize}

\blue{A preliminary version of this work has appeared in \cite{pmlr-v120-bedi20a} but the current work is a substantially improved version. Specifically, (1) the regret bounds in this work are improved and achieves sublinear regret for any $\epsilon\geq\mathcal{O}({1}/{\sqrt{T}})$ while this condition is $\epsilon\geq\mathcal{O}({1}/{{T}})$ in \citep{pmlr-v120-bedi20a}. (2) a non-asymptotic characterization of dictionary size is provided which is not present in \citep{pmlr-v120-bedi20a}, (3) all the detailed mathematical proofs of Theorems and Lemmas are included, (4) an additional analysis of EI acquisition function is added, and (5) the experimental section is improved and now includes further comparisons to other state of the art algorithms \citep{srinivas2012information,nguyen2017regret,,calandriello2019gaussian}.  }

==> Problem.tex <==
%!TEX root = main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% S  E  C  T  I  O  N %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Gaussian Process Bandits}\label{sec:prob}


{\bf \noindent Information Gain and Upper-Confidence Bound:} To find  $\bbx^*=\argmax_{\bbx\in\ccalX}f(\bbx)$ when $f$ is unknown, one may first globally approximate $f$ well, and then evaluate it at the maximizer. In order to formalize this approach, we propose to quantify how informative a collection of points $\{\bbx_u\}\subset \ccalX$ is through information gain \citep{cover2012elements}, a standard quantity that tracks the mutual information between $f$ and observations $y_u = f(\bbx_u) + \epsilon_u$ all indices $u$ in some sampling set, defined as
%
\begin{equation}\label{eq:information_gain}
%
I(\{y_u\}  ; f) = H(\{y_u\} ) - H(\{y_u\} \given f)
\end{equation}
%
where $H(\{y_u\} ) $ denotes the entropy of observations $\{y_u\} $ and $ H(\{y_u\} \given f)$ denotes the entropy conditional on $f$. For a Gaussian $\ccalN(\mu,\Sigma)$ with mean $\mu$ and covariance $\Sigma$, the entropy is given as
%
%
\begin{equation}\label{eq:entropy_gaussian}
%
 H(\ccalN(\mu,\Sigma))=\frac{1}{2}\log|2\pi e \Sigma |% and the information gain is given in closed form as
 %
\end{equation}
 %
 which allows us to evaluate the information gain in closed form as
 %
\begin{equation}\label{eq:information_gain_gaussian}
%
I(\{y_u\}  ; f) = \frac{1}{2}\log|2 + \sigma^{-2}\bbK_t |.
%
\end{equation}
%
%

Suppose we are tasked with finding a subset of $K$ points $\{\bbx_u\}_{u\leq T}$ that maximize the information gain. This amounts to a challenging subset selection problem whose exact solution cannot be found in polynomial time \citep{ko1995exact}. However, near-optimal solutions may be obtained via greedy maximization, as information gain is submodular \citep{krause2008near}. Maximizing information gain, i.e., selecting $\bbx_t = \argmax_{\bbx \in \ccalX} I(\{y_u\}  ; f) $, is equivalent to \citep{srinivas2012information}
 %
\begin{equation}\label{eq:max_variance}
%
\bbx_t = \argmax_{\bbx \in\ccalX} \sigma_{\bbX_{t-1}}(\bbx)
%
\end{equation}
%
where $\sigma_{\bbX_{t-1}}(\bbx)$ is the empirical standard deviation associated with a matrix $\bbX_{t-1}$ of data points $\bbX_{t-1}:=[\bbx_1 \; \cdots \bbx_{t-1} ]\in\reals^{d\times (t-1)}$.
%
We note that \eqref{eq:max_variance} may be shown to obtain the near-optimal selection of points in the sense that after $T$ rounds, executing \eqref{eq:max_variance} guarantees $$I(\{y_u\}_{{u=1}}^T  ; f)  \geq (1 - 1/e) I(\{y_u\}_{{u=1}}^K  ; f)$$ for some $K \leq T$ points via the theory of submodular functions  \citep{nemhauser1978analysis}. Indeed, selecting points based upon \eqref{eq:max_variance} permits one to efficiently \emph{explore} $f$ globally. However, it dictates that action selection does not move towards the actual maximizer $\bbx^*$ of $f$. For this, $\bbx_t$ should be chosen according to prior knowledge about the function $f$, \emph{exploiting} information about where $f$ is large. To balance between these two extremes, a number of different acquisition functions $\alpha(\bbx)$ are possible based on the GP posterior -- see \citep{powell2012optimal}. Here, for simplicity, we propose to do so either based upon the upper-confidence bound (UCB):
 %
\begin{equation}\label{eq:gp_ucb}
%
\bbx_t = \argmax_{\bbx \in\ccalX}\underbrace{\mu_{\bbX_{t-1}}(\bbx) + \sqrt{\beta_t} \sigma_{\bbX_{t-1}}(\bbx)}_{\alpha^{\text{UCB}(\bbx)}}
%
\end{equation}
%
with $\beta_t$ as an exploration parameter $\beta_t$, or the expected improvement (EI) \citep{nguyen2017regret}, defined as
%
\begin{equation}\label{eq:expected_improvement}
%
\bbx_t=\argmax_{\bbx\in\ccalX} \underbrace{\sigma_{t-1}\phi(z) + [\mu_{t-1}\!(\bbx) - y^{\text{max}}_{t-1}]\Phi(z)}_{\alpha^{\text{EI}(\bbx)}}\;,
%
\end{equation}
%
where $ y^{\text{max}}_{t-1}= \max\{y_u\}_{u\leq t}$ is the maximum observation value of past data, $z=z_{t-1}(\bbx) = (\mu_{t-1}(\bbx) - y^{\text{max}}_{t-1} )/\sigma_{t-1}(\bbx)$ is the $z$-score of $y^{\text{max}}_{t-1}$, and $\phi(z)$ and $\Phi(z)$ denote the density and distribution function of a standard Gaussian distribution. Moreover, the aforementioned mean $\mu_{t-1}(\bbx)$ and standard deviation $\sigma_{t-1}(\bbx)$ in the preceding expressions are computed via a GP, to be defined next. 

{\bf \noindent Gaussian Processes:} A Gaussian Process (GP) is a stochastic process for which every finite collection of realizations is jointly Gaussian. We hypothesize a Gaussian Process prior for $f(\bbx)$, which is specified by a mean function $$\mu(\bbx)=\E{f(\bbx)}$$ and covariance kernel defined as $$\kappa(\bbx, \bbx') =  \E{(f(\bbx)-\mu(\bbx))^T(f(\bbx')-\mu(\bbx') )}.$$ Subsequently, we assume the prior is zero-mean $\mu(\bbx)=0$.
%
GPs play multiple roles in this work: as a way of specifying smoothness and a prior for unknown function $f$, as well as characterizing regret when $f$ is a sample from a known GP $GP(\bb0; \kappa(\bbx; \bbx'))$. GPs admit a closed form for their conditional a posteriori mean and covariance given training set $\ccalS_t=\{\bbx_u,\bby_u\}_{u\leq t}$ as \citep{rasmussen2004gaussian}[Ch. 2]. 
%
\begin{align}\label{eq:posterior_parameters}
\mu_{\bbX_t}(\bbx)& = \bbk_t(\bbx)^T(\bbK_t + \sigma^2 \bbI)^{-1} \bby_t  \\
\sigma^2_{\bbX_t} (\bbx)& = \kappa(\bbx, \bbx')- \bbk_t(\bbx)^T(\bbK_t + \sigma^2 \bbI)^{-1} \bbk_t(\bbx')^T\nonumber
\end{align}
%
where $\bbk_t (\bbx)=[\kappa(\bbx_1, \bbx), \cdots, \kappa(\bbx_t, \bbx)] $ denotes the empirical kernel map and $\bbK_t$ denotes the gram matrix of kernel evaluations whose entries are $\kappa(\bbx, \bbx')$ for $\bbx,\bbx'\in\{\bbx_u\}_{u\leq t}$. The $\bbX_t$ subscript underscores its role in parameterizing the mean and covariance. Further, note that \eqref{eq:posterior_parameters} depends upon a linear observation model $y_t = f(\bbx_t) + \epsilon_t$ with Gaussian noise prior $\epsilon_t \sim \ccalN (0,\sigma^2)$. 
%
The parametric updates \eqref{eq:posterior_parameters} depend on past actions $\{\bbx_{u}\}_{\{u\leq t\}}$, which causes the \emph{kernel dictionary} $\bbX_t$ to grow by one at each iteration, i.e., 
%
$$\bbX_{t+1} = [\bbX_t \ ; \ \bbx_{t+1}] \in \reals^{d\times t},$$ and the posterior at time $t+1$ uses \emph{all past observations} $\{\bbx_u\}_{u\leq t}$. Henceforth, the number of columns in the dictionary is called the \emph{model order}. The GP posterior at time $t+1$ has model order $t$. 

 The resulting action selection strategy \eqref{eq:gp_ucb} using the GP \eqref{eq:posterior_parameters} is called GP-UCB, and its regret \eqref{eq:regret} is established in \citep{srinivas2012information}[Theorem 1 and 2] as sublinear with high probability up to factors depending on the maximum information gain $\gamma_T$ over $T$ points, which is defined as 
%
\begin{equation}\label{eq:max_info_gain}
%
\gamma_T:=\max_{ \{\bbx_u \} } I(\{y_u\}_{{u=1}}  ; f) \ \text{ such that } \ |\{\bbx_u \} |=T.
%
\end{equation}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
	\caption{\textcolor{black}{Compressed GP-Bandits (COB)}}\label{alg:cub}
	%
	\begin{algorithmic}
	%
		\FOR{t = 1,2...}
		%
		\STATE Select action $\bbx_{t}$ via UCB \eqref{eq:gp_ucb} or EI \eqref{eq:expected_improvement}: $$\bbx_{t} = \arg\max_{\bbx\in\mathcal{X}} \alpha(\bbx)$$\\
		 
		% We have a distribution $\hat{\mathcal{G}}_{t-1}=\mathcal{N}(\hat{\mu}_{t-1}(\bbx),\hat\sigma_{t-1}^{2}(\bbx))$
		%
		\STATE Sample: $ y_{t} = f(\bbx_{t})+\epsilon_{t}$
		%
		 \STATE{\bf If} conditional entropy exceeds $\epsilon$ threshold $\mathbf{H}(y_{t}|\bby_{t-1})=\frac{1}{2}\log\big(2\pi e(\sigma^{2}+{\sigma}^{2}_{\bbD_{t-1}}(\bbx_{t}))\big)>\epsilon$
		\INDSTATED Augment dictionary ${{\bbD}}_{t} = [{{\bbD}}_{t-1};\bbx_{t} ]$
		\INDSTATED Append $y_t$ to target vector $\bby_{\bbD_t}=[ \bby_{\bbD_{t-1}} ; y_t]$ 
			\INDSTATED Update posterior mean ${\mu}_{\bbD_t}(\bbx)$ \& variance ${\sigma}_{\bbD_t}(\bbx)$ 
		%
		\begin{align*}
		\!\!\!\!&{\mu}_{\bbD_t}(\bbx)={\boldsymbol{k}}_{{{\bbD}}_{t}}(\bbx)^{T}(\bbK_{\bbD_t}+\sigma^{2}\bbI)^{-1}\bby_{{{\bbD}}_{t}}&
		%
		\\		\!\!\!\!&\sigma_{\bbD_t}^{2}\!(\bbx)\!=\kappa(\bbx,\!\bbx^{\prime})\!-\!{\boldsymbol{k}}_{{{\bbD}}_{t}}(\bbx)^T(\bbK_{\bbD_t,\bbD_t}\!\!+\!\!\sigma^{2}\bbI)^{-1}{\boldsymbol{k}}_{{{\bbD}}_{t}}(\bbx^{\prime})
		%\\
		%\hat\sigma_{t}^{2}(\bbx)=&\kappa_{t}(\bbx,\bbx) 
				\end{align*}
				\vspace{-4mm}
		\STATE{\bf else} 
		\INDSTATED Fix dict. $\bbD_t= \bbD_{t-1}$, target $\bby_{\bbD_t}= \bby_{\bbD_{t-1}}$, \& GP.
		$$(\mu_{\bbD_t}(\bbx),{\sigma}_{\bbD_t}(\bbx),{\bbD}_{t})=(\mu_{{\bbD_{t-1}}}(\bbx),{\sigma}_{\bbD_{t-1}}(\bbx),{\bbD}_{t-1})$$
		\ENDFOR
		%
	\end{algorithmic}
	%
\end{algorithm}
{\bf \noindent Compression Statistic:} The fundamental role of information gain in the regret of GP, using either UCB or EI,  provides a conceptual basis for finding a parsimonious GP posterior that nearly preserves no-regret properties of \eqref{eq:gp_ucb} - \eqref{eq:posterior_parameters}. To define our compression rule, first we define some key quantities related to approximate GPs. Suppose we select some other kernel dictionary $\bbD\in\reals^{d\times M}$ rather than $\bbX_t$ at time $t$, where $M$ is the  \emph{model order} of the Gaussian Process. Then, the only difference is that the kernel matrix $\bbK_t$ in \eqref{eq:posterior_parameters} and the empirical kernel map $\bbk_{t}(\cdot)$ are substituted by $\bbK_{\bbD\bbD}$ and $\bbk_{\bbD}(\cdot)$, respectively, where the entries of $[\bbK_{\bbD\bbD}]_{mn}=\kappa(\bbd_m, \bbd_n)$ and $\{\bbd_m  \}_{m=1}^M \subset \{\bbx_u\}_{u\leq t}$. Further, $\bby_\bbD$ denotes the sub-vector of $\bby_t$ associated with only the indices of training points in matrix $\bbD$. We denote the training subset associated with these indices as $\ccalS_{\bbD}:=\{\bbx_u,y_u\}_{u=1}^M$. By rewriting \eqref{eq:posterior_parameters} with $\bbD$ as the dictionary rather than $\bbX_{t+1}$, we obtain
%
 \begin{align}\label{eq:GP_posterior_D}
\bbmu_{\bbD}(\bbx)&=\bbk_{\bbD}(\bbx_{t+1})[\bbK_{\bbD,\bbD}+ \sigma^2 \bbI]^{-1}\bby_{\bbD}  \\
%
\sigma_{\bbD}^{2}(\bbx)=&\kappa(\bbx,\bbx^{\prime})-{\boldsymbol{k}}_{{\bbD}}(\bbx)^T(\bbK_{\bbD,\bbD}+\sigma^{2}\bbI)^{-1}{\boldsymbol{\kappa}}_{\bbD}(\bbx^{\prime}).\nonumber
 \end{align}
 %
The question, then, is how to select a sequence of dictionaries $\bbD_t \in \reals^{p\times M_t}$ whose $M_t$ columns comprise a subset of those of $\bbX_t$ in such a way to approximately preserve the regret bounds of \citep{srinivas2012information}[Theorem 1 and 2] while ensuring the model order is moderate $M_t \ll t$.

% Clearly, information gain [cf. \eqref{eq:information_gain}] plays a fundamental role in Gaussian Process bandits, as the maximum over a collection of points $\{\bbx_u\}$ \eqref{eq:max_info_gain} appears as a fundamental quantifier of learning performance (Lemma \ref{lemma:template}. Thus, 
 
We propose using conditional entropy as a statistic to compress against, i.e., a new data point should be appended to the Gaussian process posterior only when its conditional entropy is at least $\epsilon$, which results in the following update rule for the dictionary $\bbD_{t} \in \reals^{p\times M_t }$:
%
\begin{align}\label{eq:compression_rule}
%
 &\textbf{If } \ \mathbf{H}(y_{t}|\hat\bby_{t-1})=\frac{1}{2}\log\big(2\pi e(\sigma^{2}+{\sigma}^{2}_{\bbD_{t-1}}(\bbx_{t}))\big)>\epsilon \nonumber \\ 
&\ \ \ \  \text{update} \ \ \ \bbD_{t} =[\bbD_{t-1} \ ; \ \bbx_{t}]\nonumber \\
&\textbf{else } \nonumber \\
& 
\ \ \ \  \text{update} \ \ \ \bbD_{t}= \bbD_{t-1} ,
%
\end{align}
%
where we define $\epsilon$ as the compression budget. This amounts to a statistical test of whether the action $\bbx_t$ yielded an informative sample $y_t$ in the sense that its conditional entropy exceeds an $\epsilon$ threshold. Therefore, uninformative past decisions are dropped from belief formation about the present. The modification of GP-UCB, called \emph{Compressed GP-UCB}, or \emph{CUB} for short, uses \eqref{eq:gp_ucb} with the lazy GP belief model \eqref{eq:GP_posterior_D} defined by dictionary updates \eqref{eq:compression_rule}. Similarily, the compression version of EI is called Compressed EI or CEI for short. We present them together for simplicity as Algorithm \ref{alg:cub} with the understanding that in practice, one must specify UCB \eqref{eq:gp_ucb} or EI \eqref{eq:expected_improvement}.
%%
%
Next, we rigorously establish how Algorithm \ref{alg:cub} trades off regret and memory through the $\epsilon$ threshold on conditional entropy for whether a point $(\bbx_t, y_t)$ should be included in the GP.



 
